Learning Transferable Reward for Query Object Localization with Policy Adaptation

We propose a reinforcement learning based approach to query object localization, for which an agent is trained to localize objects of interest specified by a small exemplary set. We learn a transferable reward signal formulated using the exemplary set by ordinal metric learning. Our proposed method enables test-time policy adaptation to new environments where the reward signals are not readily available, and outperforms fine-tuning approaches that are limited to annotated images. In addition, the transferable reward allows repurposing the trained agent from one specific class to another class. Experiments on corrupted MNIST, CU-Birds, and COCO datasets demonstrate the effectiveness of our approach.

==> ICLR2022_Policy Adaptation_Final/abstract.tex <==

%We propose a reinforcement learning based approach to the problem of \emph{query object localization}, where an agent is trained to localize objects of interest specified by a small exemplary set. We learn a transferable reward signal formulated using the exemplary set by ordinal metric learning. It enables test-time policy adaptation to new environments where the reward signals are not readily available, and outperforms fine-tuning approaches that are limited to annotated images.  In addition, the transferable reward can allow repurposing of the trained agent from one specific class to another class. Experiments on corrupted MNIST, CU-Birds, and COCO datasets demonstrate the effectiveness of our approach. 

We propose a reinforcement learning based approach to \emph{query object localization}, for which an agent is trained to localize objects of interest specified by a small exemplary set. We learn a transferable reward signal formulated using the exemplary set by ordinal metric learning. Our proposed method enables test-time policy adaptation to new environments where the reward signals are not readily available, and outperforms fine-tuning approaches that are limited to annotated images.  In addition, the transferable reward allows repurposing the trained agent from one specific class to another class. Experiments on corrupted MNIST, CU-Birds, and COCO datasets demonstrate the effectiveness of our approach \footnote{Code available at \url{https://github.com/litingfeng/Localization-by-OrdEmbed}}. 

% In addition, the transferable reward can allow repurposing of the trained agent for new tasks, {\color{red}such as annotation refinement, or selective localization from multiple common objects across a set of images.} Experiments on corrupted MNIST dataset and CU-Birds dataset {\color{red}and MS COCO?} demonstrate the effectiveness of our approach. 

==> ICLR2022_Policy Adaptation_Final/acknowledgement.tex <==
This research has been partially funded by the following grants 
ARO MURI 805491, NSF IIS-1793883, NSF CNS-1747778, NSF IIS 1763523, DOD-ARO ACC-W911NF, NSF OIA-2040638 to D. Metaxas. 
We would like to thank anonymous reviewers for their
comments and suggestions.

==> ICLR2022_Policy Adaptation_Final/discussion.tex <==
We propose an ordinal representation learning based reward, for training a localization agent to search queried objects of interest. In particular, we use a small exemplary set as a guidance signal for delivering learning objectives without ambiguity. Meanwhile, we use test image environments to inform the agent about the domain shifts, without requiring image-box pairs during %the 
test time. 

 Instead of jointly training a localization and classification model, we learn box annotations from image class labels, in a similar spirit %with  
 to weakly-supervised learning.  Empirically, we focus extensively on the \emph{transfer learning} setting from one single data abundant training task to data-scarce (one-way few-shot) test tasks \citep{taylor2009transfer, zhu2020transfer}. %In making
 To make a trained RL agent generalizable to new unseen test cases, one can either expose the agent to as many cases as possible during training, or make the agent more specific but adaptable upon changed scenarios. Our approach belongs to the latter. 
 
 % It shows that even if only one training class is accessible, the agent with transferable reward can still adapt to various cases during the test time.
 
 % Appendix: Our approach is also applicable to the many-way few-shot setting where limited annotations across multiple classes are available during training.

The transferability of our reward signal from training to test crucially relies on the generalization ability of the learned ordinal representation. If the ordinal preference does not hold in the test domain, the proposed test-time policy adaptation scheme will not work. By adapting the representation with self-supervised objectives \citep{hansen2021selfsupervised}, this issue might be remedied. 


% We left it as future work. 

Although our work focuses on the generalization ability of a single object localizer, extensions to multiple objects can possibly be done by applying it multiple times and marking the found regions, in a similar manner as \citep{caicedo2015active}. Curriculum learning with a designed sequence of targets in the exemplary set may guide the agent toward solving challenging localization tasks. We leave those extensions for future study. 



% Although our approach focuses on object localization of a single object, extensions to multiple objects can be doable. 

% Although our approach does not directly handle the special cases of multiple queried objects or no queried object within the image environment, it can be {\color{red}easily modified} to accomplish these tasks. %



% Appendix: Annotation collection plays an important role in building machine learning systems. It is one task that could benefit greatly from automation, especially in cost-sensitive applications. We aim to reduce the human labeling efforts, in terms of the number of annotate samples per class, number of annotate classes (one-class at the minimum), and the level of accuracy required, all under the same query-adaptation framework.  


% and we leave it for future study.  





% We leave the robustness to bias and vulnerability to adversarial attacks for future study. 

% %%% Before 1121
% We propose an ordinal representation learning based reward, for training a localization agent to search queried object of interest. In particular, we use a small exemplary set as a guidance signal for delivering learning objectives, which can avoid potential learning ambiguity. Meanwhile, we use test image environments to inform the agent about the domain shifts, without requiring image-box pairs during the test-time. 



% The transferability of our reward signal from training to testing crucially relies on the generalization ability of the learned ordinal representation. If the ordinal preference does not hold in the test domain, the proposed test-time policy adaptation scheme will not work. By adapting the representation with self-supervised objectives \citep{hansen2021selfsupervised}, this issue might be remedied. We left it as future work. Although our approach does not directly handle the special cases of multiple queried objects or no queried object within the image environment, it can be {\color{red}easily modified} to accomplish these tasks. %



% Annotation collection plays an important role in building machine learning systems. It is one task that could benefit greatly from automation, especially in cost-sensitive applications. We aim to reduce the human labeling efforts, in terms of the number of annotate samples per class, number of annotate classes (one-class at the minimum), and the level of accuracy required, all under the same query-adaptation framework. Instead of jointly training the localization and classification model, we learn box annotations from image class labels, in a similar spirit with weakly-supervised learning.  Empirically, we focus extensively on the \emph{transfer learning} setting from one single data abundant training task to data-scarce (one-way few-shot) test tasks. Our approach is also applicable to the many-way few-shot setting where limited annotations across multiple classes are available during training, and we leave it for future study.  


% In making the trained RL agent generalizable to new unseen test cases, one can either expose the agent to as many cases as possible during training, or make the agent more specific but adaptable upon changed scenarios. Our approach belongs to the latter, which shows that even if only one training class is accessible, the agent with transferable reward can still adapt to various cases during the test time. As an extension work, curriculum learning with a designed sequence of targets in the exemplary set may guide the agent toward solving challenging localization tasks. We leave the robustness to bias and vulnerability to adversarial attacks for future study. 

% ------------

% We propose an ordinal representation learning based reward, for training a localization agent to search queried object of interest. In particular, we use a small exemplary set as a guidance signal for delivering learning objectives, which can avoid potential learning ambiguity. Meanwhile, we use test image environments to inform the agent about the domain shifts, without requiring image-box pairs during the test-time. 



% The transferability of our reward signal from training to testing crucially relies on the generalization ability of the learned ordinal representation. If the ordinal preference does not hold in the test domain, the proposed test-time policy adaptation scheme will not work. By adapting the representation with self-supervised objectives \citep{hansen2021selfsupervised}, this issue might be remedied. We left it as future work. Although our approach does not directly handle the special cases of multiple queried objects or no queried object within the image environment, it can be {\color{red}easily modified} to accomplish these tasks. %


% % In many applications, the object of interest is specific. 

% % For example, in digital pathology, localizing one particular type of cancer cells from slides collected from one hospital, and adapt to slides collected by different scanning machines, different staining, or from different organs.



% % MS COCO dataset has high inter-class heterogeneity. It is a good while challenging dataset for class-agnostic and few-shot object detection/localization methods. These models are trained with abundant classes in order to generalize to various new classes. We think the CUB dataset might be more suitable to evaluate the transfer learning setting since it has a certain discrepancy between classes and species but they still have to be related.



 

% % Given an image label from a classification model, our localization model can identify the box region with enhanced interpretability.

% % Our approach can enhance interpretability of classification as a post-processing step.


% Annotation collection plays an important role in building machine learning systems. It is one task that could benefit greatly from automation, especially in cost-sensitive applications. We aim to reduce the human labeling efforts, in terms of the number of annotate samples per class, number of annotate classes (one-class at the minimum), and the level of accuracy required, all under the same query-adaptation framework. Instead of jointly training the localization and classification model, we learn box annotations from image class labels, in a similar spirit with weakly-supervised learning.  Empirically, we focus extensively on the \emph{transfer learning} setting from one single data abundant training task to data-scarce (one-way few-shot) test tasks. Our approach is also applicable to the many-way few-shot setting where limited annotations across multiple classes are available during training, and we leave it for future study.  





% In making the trained RL agent generalizable to new unseen test cases, one can either expose the agent to as many cases as possible during training, or make the agent more specific but adaptable upon changed scenarios. Our approach belongs to the latter, which shows that even if only one training class is accessible, the agent with transferable reward can still adapt to various cases during the test time. As an extension work, curriculum learning with a designed sequence of targets in the exemplary set may guide the agent toward solving challenging localization tasks. We leave the robustness to bias and vulnerability to adversarial attacks for future study. 


% cross-modality retrieval or zero-shot query based on attributes, and





% (1) One class, abundant 
% (2) Orthogonal, multiple class, few-shot classification --> few-shot localization 
% (3) Few-shot/WSOL classification + One class, abundant, policy on class A --> class B, C, D

% Localization -> Classification 

% Jointly Localization + Classification 
% Ours: classification -> Localization




% use exemplary set as a guidance signal for deliver learning objectives 

% use test image environment to expose the agent to the domain shifts 

% taking raw image pixel as input


% with improved generalization and adaptation abilities during test-time.   



% fundamentally different with bounding-box regression, object detection methods, focus different. 


% \paragraph{Broader Impact} 






==> ICLR2022_Policy Adaptation_Final/experiment.tex <==
% We evaluate ... across three different angles. First, we consider synthetic task . Next, we experiment . Lastly, we demonstrate performance on. 
% successfully
% adapt agent policies to substantial changes,
 
% Computation. Tricks that works.
In this section, we evaluate the generalization ability of the ordinal embedding as well as the performance of the trained localization agent on both source and target domains. 
The embedding-based
reward not only improves the RL training, but also enables test-time adaptation of the learned policy.
Experimental results demonstrate the effectiveness of our approach, with empirical comparisons to fine-tuning, co-localization, few-shot and Faster RCNN object detection baselines.
  
% We also explore test-time policy adaptation on novel tasks such as \emph{annotation refinement} and \emph{selective localization}.

% \paragraph{Baselines.} For RL object localization, we compare the proposed method with the IoU reward based DeepQNetwork methods \citep{caicedo2015active, jie2016tree}.  Besides the differences discussed in Section \ref{sec: limitations},  differences in the RL implementation (e.g., reward and policy learning method) are also compared empirically. For policy adaptation, we compared our policy adaptation scheme with a standard fine-tuning scheme on the policy network. 

% {\color{red}  DDT baseline, }
% {\color{red}  few-shot object detection baseline}

\textbf{Implementation details.} To evaluate the learned ordinal embedding, we use \emph{OrdAcc} defined as the percentage of images within which the preference between a pair of perturbed boxes is correctly predicted. To evaluate object localization performance, we use the Correct Localization (\emph{CorLoc}) \citep{deselaers2012weakly} metric, which is defined as the percentage of images correctly localized according to the criterion $\textrm{IoU}(b_{p}, g)\geq 0.5$, where $b_{p}$ is the predicted box and $g$ is the ground-truth box. Mean and standard deviation (displayed as subscript) are reported from {\color{black}$10$} independent runs. We evaluate our approach on distorted versions of the MNIST handwriting, the CUB-200-2011 birds \citep{wah2011caltech}, and the COCO \citep{lin2014microsoft} dataset. For the MNIST dataset, we use three convolutional layers with ReLU activation after each layer as the image encoder. For the CUB and the COCO datasets, we adopt layers before \emph{conv5\_3} of VGG-16 pre-trained on ImageNet %for
as the encoder, unless otherwise specified. More details are presented in Appendix \ref{app:imp}.

% (unless mentioned elsewise).
% $\textrm{area}(b_{p}\cap g)}/{\textrm{area}(b_{p}\cup g)}\geq 0.5$

\vspace{-0.2cm}
\subsection{Policy adaptation during test time}

We demonstrate the performance improvement with test-time policy adaptation. Through all the experiments, we assume source domain contains abundant data annotations, and target domain annotations are only available in an exemplary set of size $5$. We compare our policy adaptation scheme with a standard fine-tuning scheme on the pre-trained policy network.

\textbf{Results on the corrupted MNIST dataset.} For the new class adaptation experiment, we use 50 ``digit $4$ images under random patch background noises" to train the ordinal embedding and the localization agent. % \sout{During test time, either the class of the foreground object or the background changes.} 
The results on policy adaptation to \emph{new digits} (other than $4$) are shown in Table \ref{tab:mnist-class}. Row $1$ illustrates the transferability of the ordinal embedding reward,  trained prototype embedding of a subgroup without the training instance,  and evaluated using instance embedding  from the same test image (``$OrdAcc$"). Rows $2$ to $4$ list the resulting localization accuracy after direct generalization (``before"), fine-tuning on the exemplary set (``fine-tune"), and adaptation using all test images (``adapt"), respectively. Our policy adaptation approach  produces a substantial improvement over direct generalization, while fine-tuning approach experiences overfitting on the limited exemplary set. For the background adaptation experiment, we train on 50 digit-3 images under random patch noise, and test on digit-2 images under all four noises. The localization accuracy on both source and \emph{new backgrounds} environment are shown in Table \ref{tab:mnist-background}, significant improvements are achieved using our policy adaptation scheme.      
%  The resulting localization accuracy after direct generalization, fine-tuning on the exemplary set, and adaptation using {\color{red}$50$} test images are listed in the third, fourth, and fifth row, respectively.
\begin{table}[ht]
\tiny
\vspace{-0.2cm}
\setlength{\tabcolsep}{2pt}
\centering
\caption{{\color{black}$OrdAcc$ (\%)} and  $CorLoc$ (\%) on new digits environment.}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}[t]{lccccccccccc}
\toprule
& 0 & 1 & 2 & 3& 5 & 6 & 7 & 8 & 9 & mean   \\
\midrule
% Ord SP   & $89.4_{0.6}$ & $88.2_{3.0}$ & $90.8_{2.2}$ & $90.3_{1.2}$ & $90.7_{0.4}$ & $91.1_{1.8}$ & $89.3_{0.9}$ & $90.8_{0.5}$ & $89.3_{0.7}$ & $90.0_{0.7}$ \\
$OrdAcc$  & $91.9_{0.7}$ & $90.3_{2.9}$ & $92.1_{1.8}$ & $92.0_{0.2}$ & $92.7_{0.6}$ & $92.6_{0.2}$ & $90.7_{0.7}$ & $92.0_{0.7}$ & $90.5_{0.7}$ & $91.6_{0.5}$ \\
\midrule
before & $94.2_{0.6}$ & $84.1_{1.5}$ & $88.7_{1.7}$ & $86.5_{1.8}$ & $81.2_{1.4}$ & $91.9_{0.3}$ & $ 89.5_{0.7}$ & $93.0_{1.0}$ & $90.8_{0.4}$ & $88.9_{1.0}$ \\
fine-tune & $93.3_{2.5}$ & $80.4_{3.9}$ & $84.5_{3.5}$ & $84.9_{1.5}$ & $ 78.8_{2.7}$ & $87.3_{2.9}$ &  $82.2_{5.4}$ & $87.7_{4.5}$ & $85.6_{5.3}$ & $83.7_{4.5}$ \\
adapt & $99.8_{0.2}$ & $95.6_{0.6}$ & $98.1_{0.4}$ & $97.9_{0.4}$ & $88.3_{0.5}$ & $99.1_{0.2}$ & $98.6_{0.9}$ & $99.8_{0.3}$ & $99.2_{0.4}$ & $97.4_{0.4}$ \\
\bottomrule
\end{tabular}
}
% \vspace{-0.6cm}
\label{tab:mnist-class}
\end{table}%


% \begin{table}[ht]
% \tiny
% \vspace{-0.3cm}
% \setlength{\tabcolsep}{2pt}
% \centering
% \caption{{\color{red}$OrdAcc$ (\%)} and  $CorLoc$ (\%) on new digits environment.}
% \resizebox{0.99\textwidth}{!}{
% \begin{tabular}[t]{lccccccccccc}
% \toprule
% & 0 & 1 & 2 & 3& 5 & 6 & 7 & 8 & 9 & average   \\
% \midrule
% % Ord SP   & $89.4_{0.6}$ & $88.2_{3.0}$ & $90.8_{2.2}$ & $90.3_{1.2}$ & $90.7_{0.4}$ & $91.1_{1.8}$ & $89.3_{0.9}$ & $90.8_{0.5}$ & $89.3_{0.7}$ & $90.0_{0.7}$ \\
% Ord Inst  & $91.9_{0.7}$ & $90.3_{2.9}$ & $92.1_{1.8}$ & $92.0_{0.2}$ & $92.7_{0.6}$ & $92.6_{0.2}$ & $90.7_{0.7}$ & $92.0_{0.7}$ & $90.5_{0.7}$ & $91.6_{0.5}$ \\
% \midrule
% before & $94.2_{0.6}$ & $84.1_{1.5}$ & $88.7_{1.7}$ & $86.5_{1.8}$ & $81.2_{1.4}$ & $91.9_{0.3}$ & $ 89.5_{0.7}$ & $93.0_{1.0}$ & $90.8_{0.4}$ & $88.9_{1.0}$ \\
% finetune & $93.3_{2.5}$ & $80.4_{3.9}$ & $84.5_{3.5}$ & $84.9_{1.5}$ & $ 78.8_{2.7}$ & $87.3_{2.9}$ &  $82.2_{5.4}$ & $87.7_{4.5}$ & $85.6_{5.3}$ & $83.7_{4.5}$ \\
% adapt & $99.8_{0.2}$ & $95.6_{0.6}$ & $98.1_{0.4}$ & $97.9_{0.4}$ & $88.3_{0.5}$ & $99.1_{0.2}$ & $98.6_{0.9}$ & $99.8_{0.3}$ & $99.2_{0.4}$ & $97.4_{0.4}$ \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-0.6cm}
% \label{tab:mnist-class}
% \end{table}%

% \begin{table}[bpht]
% \centering
% \caption{$CorLoc$ (\%) when transferring to other background.}
% \small{
% \begin{tabular}[t]{cccccc}
% \toprule
% Adaption &  random patch & clutter & impulse noise & Gaussian noise & average\\
% \midrule
% & 97.67 & 39.05 & 22.77 & 68.99 & 57.12\\
% \checkmark& \textbf{100.00} & \textbf{97.67} & \textbf{100.00} & \textbf{100.00} & \textbf{99.42} \\
% \bottomrule
% \end{tabular}}
% \label{tab:mnist-background2}
% \vspace{-0.3cm}
% \end{table}


\begin{table}[bpht]
\vspace{-0.2cm}
\centering
\caption{$CorLoc$ (\%) when adapted to other background on corrupted MNIST dataset.}
\small{
\begin{tabular}[t]{cccccc}
\toprule
adapt &  random patch & clutter & impulse noise & gaussian noise & mean \\
\midrule
& $97.6_{0.4}$ & $39.6_{0.5}$ & $22.1_{0.7}$ & $66.2_{2.0}$ & $56.4$ \\
\checkmark& $\mathbf{100.0}_{\mathbf{0.0}}$ & $\mathbf{97.4}_{\mathbf{0.3}}$ & $\mathbf{99.9}_{\mathbf{0.1}}$ & $\mathbf{100.0}_{\mathbf{0.0}}$ &  
$\mathbf{99.3}$ \\
\bottomrule
\end{tabular}}
\label{tab:mnist-background}
\vspace{-0.0cm}
\end{table}



\textbf{Results on the CUB dataset.} We also evaluate the policy adaptation performance on the CUB dataset. The localization agent is trained on $15$ species from the ``Warbler" class, and adapted to different classes of ``Warbler" ($5$ new species), ``Wren", ``Sparrow", ``Oriole", ``Kingfisher", ``Vireo", and ``Gull". Each test class contains a single bird class. We also implement deep descriptor transforming (DDT) \citep{wei2017deep}, a deep learning based co-localization approach, and add it to the comparison. 
% {\color{red}Our test-time policy adaptation scheme yields $2.81\%$ and $8.36\%$ improvement of localization accuracy on average.Numbers look not correct. Maybe remove this whole sentence.} 

% \begin{table}[bpht]
% \small
% \centering
% \vspace{-0.3cm}
% \caption{$CorLoc$ when adapted to other classes on CUB dataset. Exemplary size =5.}
% \begin{tabular}[t]{ccccccccc}
% \toprule
% Adaption &  Warbler (new) & Wren & Sparrow & Oriole & Kingfisher & Vireo & Gull & Mean \\
% \midrule
% & 83.67 & 82.94 & 83.47 & 78.24 & 78.33 & 86.55 & 88.02 & 83.03\\
% \checkmark& \textbf{87.76} & \textbf{91.30} & \textbf{86.28} & \textbf{84.10} &\textbf{83.33} & \textbf{89.73} & \textbf{93.31} & \textbf{87.97} \\
% \bottomrule
% \end{tabular}
% \vspace{-0.3cm}
% \label{tab:trs2}
% \end{table}


\begin{table}[bpht]
%\small
\vspace{-0.2cm}
\centering
\caption{$CorLoc$ (\%) when adapted to other species/classes on CUB dataset.}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}[t]{lccccccccc}
% \begin{tabular}[t]{p{0.10\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.06\textwidth}}%{ccccccccc} %%{ccccccccc}{p{0.1\textwidth}}
\toprule
& adapt &  warbler (new) & wren & sparrow & oriole & kingfisher & vireo & gull & mean \\
\midrule
DDT & & 73.8 & 78.6 & 71.2 & 74.5 & 78.0 & 69.2 & 93.3 & 76.9 \\
\rowcolor{gray!10} 
& & $85.5_{1.1}$& $82.9_{2.6}$ & $81.3_{3.7}$ & $77.9_{0.7}$ &$78.9_{0.6}$ & $82.2_{4.6}$ & $86.3_{3.5}$ & $82.1$  \\
\rowcolor{gray!10}
\multirow{-2}{*}{Ours} & \checkmark&  $\mathbf{89.7}_{\mathbf{1.1}}$& $\mathbf{91.0}_{\mathbf{1.1}}$ & $\mathbf{89.3}_{\mathbf{1.8}}$ &  $\mathbf{85.0}_{\mathbf{0.8}}$ & $\mathbf{85.9}_{\mathbf{4.4}}$ & $\mathbf{90.0}_{\mathbf{0.9}}$ & $\mathbf{93.9}_{\mathbf{0.5}}$ & 
 $\mathbf{89.3}$ \\
\bottomrule
\end{tabular}}
% \vspace{-0.1cm}
\label{tab:trs}
\end{table}

\textbf{Results on the COCO dataset.} Given a target domain that one would like to deploy models to, a natural question is whether one should collect labeled data from an abundant number of source domains or from one specific class with potential lower data collection cost. On the COCO dataset, we train on one of the five classes: \emph{cat, cow, dog, horse, zebra}, then adapt to another four classes. The results are shown in Figure \ref{fig:coco}. The models perform best using ordinal embedding reward with adaptation (see ``ours-adapt"). It shows that, %despite that
although an agent is trained in a highly specialized way on only one-source tasks, it can still be flexibly generalized to different target tasks. One interesting observation is that, it is easy to transfer from other four classes to zebra, but not vice versa. A possible explanation might be that, 
the embedding net is biased on textures, %while
and texture information is less adaptable than shape information.
% ################################################

%\subsection{\textcolor{red}{TRANSFER FROM  SPECIFIC TO SPECIFIC}}
% \subsection{Transferable Reward Repurposing}

% \subsection{Transfer Learning vs. Few-shot Learning}
\vspace{-0.2cm}
\subsection{Comparison to few-shot object detectors}


%Given a target domain, one would like to deploy models to, a natural question arises on whether one should collect labeled data from an abundant number of source domains, or one specific class with potential lower data collection cost.

Few-shot object detection \citep{kang2019few, yan2019meta, wang2019meta, wang2020frustratingly} methods are similar to our work in adapting models to a new test case with the help of limited annotations, but they have a different requirement on the number of training classes. Being different in the generalization mechanism, %these methods
they usually require multiple classes in both stages of training and fine-tuning. On the COCO dataset, we compared the performance of our methods with TFA \citep{wang2020frustratingly}, and Meta-RCNN \citep{yan2019meta}, on the same \emph{one-way 5-shot} test setting. TFA adopts two-stage finetuning of object detector, while Meta-RCNN incorporates additional meta-learner to acquire class-level meta knowledge for generalization to novel classes. These two few-shot baselines are trained on $60$ base classes and fine-tuned on all $80$ classes, while our model is trained from one single class of the  $5$ classes randomly selected  from the base classes set: \emph{elephant, sheep, giraffe, laptop} and \emph{suitcase}. Table \ref{tab:coco} shows that with ordinal embedding, our agent achieves better performance even without adaptation, and the performance can be further improved after adaptation.




 % {\color{red}Bias of aspect ratio, in worst case, policy adaptation bring no additional benefit than training from the scratch.}...{\color{red}{setting}}
\begin{figure}[t]
  \centering
  \includegraphics[height=5.1cm,width=0.90\textwidth]{images/coco_re_v4_all_crop.pdf}
  \caption{{\color{black}$CorLoc$ (\%) Comparison with IoU-based reward on COCO dataset. ``ours": ordinal embedding based reward; ``iou": IoU based reward, ImageNet pre-trained embedding. Dotted lines are the results of directly training on target class, using embedding based reward but from a ImageNet pre-trained model, indicating the advantage of our approach, with ordinal embedding learned from a single source class and policy adaptation.}}
  \label{fig:coco}
\end{figure}

% \begin{table}[htb]
% \tiny
% \setlength{\tabcolsep}{2pt}
% \centering
% \caption{$CorLoc (\%)$ when adapted to other classes on COCO dataset.}
% \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{lcccc|cccc|cccc|cccc|cccc}
% \toprule
% source  & \multicolumn{4}{c}{zebra} & \multicolumn{4}{c}{horse} & \multicolumn{4}{c}{cat} & \multicolumn{4}{c}{dog} & \multicolumn{4}{c}{cow} \\
% target  & horse & cow   & cat   & dog   & zebra & cow   & cat   & dog   & horse & cow & dog & zebra & horse & cow & cat & zebra & horse & cat   & dog   & zebra\\
% \midrule
% iou-before  &       &       &       &       &       &       &       &       &       &     &     &       &       &     &     &   & &&&    \\
% iou-adapt &       &       &       &       &       &       &       &       &       &     &     &       &       &     &     &  &&&&\\
% \rowcolor{gray!10} 
% ours-before & 4.2 & 4.9 & 6.8 & 5.0 & 66.8 & 59.5 & 44.3 & 40.4 & 33.3 & 51.6 & 47.8 & 57.9 & 41.5 & 54.6 & 57.9 & 35.3 & 47.8 & 39.8 & 37.3 &    \\
% \rowcolor{gray!10} 
% ours-adapt & 39.2 & 33.8 & 35.7 & 16.9 & 72.8 & 64.8 & 53.4 & 44.4 & 52.1 & 56.9 & 48.9 & 67.3 & 55.9 & 62.9 & 62.8 & 63.9 & 54.2 & 46.4 & 42.3 & \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:trs-coco}
% \end{table}

\begin{table}[htb]
\vspace{-0.15cm}
\centering
\caption{$CorLoc$ (\%) Adaptation comparison with other methods on COCO dataset. "TFA w/ fc": TFA with a cosine similarity based box classifier; "TFA w/ cos":  TFA with a normal FC-based classifier; "FRCN+ft-full": Meta-RCNN with Faster RCNN as detector and finetuning both the feature extractor and the box predictor.}
\begin{tabular}{lccccc}
\toprule
target       & cat                  & dog                  & cow                  & horse  & mean  \\
\midrule
FRCN+ft-full \citep{yan2019meta} & 13.1 & 3.1 & 3.7 & 7.4 & 6.8 \\
TFA w/ fc \citep{wang2020frustratingly}  & 29.1 & 13.0 & 5.0 & 10.7 & 14.4 \\
TFA w/ cos \citep{wang2020frustratingly} & 28.0 & 10.3 & 4.5 & 8.9 & 12.9 \\
\rowcolor{gray!10} 
Ours-before & 23.0 & 20.6 & 24.5 & 21.2 & 22.3 \\
\rowcolor{gray!10} 
Ours-adapt & 40.3 & 33.5 & 43.1 & 40.2 & 39.3 \\
\bottomrule
\end{tabular}
\label{tab:coco}
\end{table}
\vspace{-0.2cm}
\subsection{Compare with supervised baseline - Faster RCNN}
We compare our framework with a strong supervised object localization baseline, Faster RCNN \citep{ren2016faster}. Both methods are trained in one class (foreground \emph{vs.} background as the classification labels in Faster RCNN) and adapted to a different class. We fine-tune the pre-trained VGG-16 model and test on each of the five classes: \emph{cow, cat, dog, horse, zebra}. The results on source domain are shown in Table \ref{tab:fastersource}. It shows that Faster RCNN can also be made into a class-specific model and it still yields superior performance on source domain.  On the target domain, we fine-tune Faster RCNN using only query set for each target class. The results are shown in Table \ref{tab:fastfinetune}. It can be seen that our method works better on new classes with test-time adaptation over the traditional fine-tuning of Faster RCNN. Note that fine-tuning requires image-box pairs in the target domain while our policy adaptation approach does not. 



\begin{table}[htp]
\centering
\caption{$CorLoc$ (\%) comparison with Faster RCNN on source domain.}
\begin{tabular}{lccccc}
\toprule
method       & cow & cat & dog & horse & zebra  \\
\midrule
Faster RCNN \citep{ren2016faster} & 70.37 & 89.82 & 85.81 & 92.65 & 85.71 \\
ours  & 70.37 & 68.46 & 61.26 & 61.28 & 79.36 \\
\bottomrule
\end{tabular}
\label{tab:fastersource}
\end{table}

\vspace{-0.15cm}
\begin{table}[h]
\small
\centering
\caption{$CorLoc$ (\%) comparison with Faster RCNN fine-tuned on target domain.}
\begin{tabular}{l|cc|cc}
\toprule
& \multicolumn{1}{c}{before fine-tune} & \multicolumn{1}{c|}{before adapt} & \multicolumn{1}{c}{after fine-tune} & \multicolumn{1}{c}{after adapt} \\
\midrule
& Faster   RCNN                       & ours             & Faster   RCNN                      & ours                            \\
\midrule
cat   -\textgreater horse   & 20.93                               & \textbf{33.32}                           & 37.73                              & \textbf{51.89}                           \\
cow   -\textgreater horse   & \textbf{54.79}                               & 48.41                           & \textbf{68.04}                              & 46.80                           \\
cog   -\textgreater horse   & 38.52                               & \textbf{41.50}                           & \textbf{58.01}                              & 55.89                           \\
zebra   -\textgreater horse & 1.12                                & \textbf{10.29}                            & 6.04                               & \textbf{39.22}                           \\
cat   -\textgreater cow     & 40.52                               & \textbf{50.85}                           & 58.55                              & \textbf{58.58}                           \\
dog   -\textgreater cow     & 54.55                               & \textbf{54.63}                           & \textbf{70.11}                              & 62.86                           \\
horse   -\textgreater cow   & \textbf{72.11}                               & 59.52                          & \textbf{75.35}                              & 64.83                           \\
zebra   -\textgreater cow   & 1.23                                & \textbf{8.14}                            & 5.86                               & \textbf{35.56}                           \\
cow   -\textgreater cat     & \textbf{46.12}                               & 39.84                           & \textbf{53.85}                              & 46.42                           \\
dog   -\textgreater cat     & \textbf{67.62}                               & 57.97                            & \textbf{77.07}                              & 63.12                           \\
horse   -\textgreater cat   & 36.67                               & \textbf{44.25}                          & 36.67                              & \textbf{53.39}                           \\
zebra   -\textgreater cat   & 0.55                                & \textbf{10.45}                            & 4.09                               & \textbf{35.73}                           \\
cat-\textgreater   dog      & \textbf{58.98}                               & 47.81                           & \textbf{66.50}                               & 48.94                           \\
cow   -\textgreater dog     & \textbf{45.85}                               & 37.28                           & \textbf{51.69}                              & 42.33                           \\
horse   -\textgreater dog   & \textbf{41.04}                               & 39.07                           & \textbf{47.69}                              & 44.77                           \\
zebra   -\textgreater dog   & 0.68                                & \textbf{7.74}                            & 3.4                                & \textbf{17.73}                           \\
cat   -\textgreater zebra   & 10.64                               & \textbf{57.58}                           & 37.97                              & \textbf{70.28}                           \\
cow   -\textgreater zebra   & 4.42                                & \textbf{39.64}                            & 19.64                              & \textbf{65.80}                           \\
dog   -\textgreater zebra   & 2.29                                & \textbf{35.27}                            & 15.88                              & \textbf{63.91}                           \\
horse   -\textgreater zebra & 7.86                                & \textbf{66.82}                          & 29.3                               & \textbf{72.83}     \\
\midrule
mean & 30.32$\pm$25.0 & \textbf{39.51$\pm$17.9} & 41.17$\pm$25.3 & \textbf{52.04$\pm$13.9} \\
\bottomrule
\end{tabular}
\label{tab:fastfinetune}
\end{table}

\vspace{-0.2cm}
\subsection{Ablation studies}\label{sec: ablation_study}
%\paragraph{Ordinal embedding and RL.}
We analyze the effectiveness of ordinal embedding and RL component separately on COCO dataset (Appendix \ref{ap:allab} provides more in-depth analysis on the corrupted MNIST dataset, including policy gradient \emph{vs.}  deep Q-Network, continuous \emph{vs.} binary reward). First, we remove RL, and substitute it with a simple linear search approach.  Specifically, we adopt selective search \citep{uijlings2013selective} for candidate boxes generation. The candidate boxes are ranked according to their embedding distances to the prototype, and the one with the smallest embedding distance is returned as the final output.  We consider two backbone networks as the embedding, including ImageNet pre-trained VGG-16 and Faster RCNN VGG-16 trained locally on COCO dataset. We also compare both with and without the ordinal component, making it a $2\times 2$ ablation study. It can be seen from the blue and green bars from Figure \ref{fig:faster_rank} and Appendix Figure \ref{fig:imgnet_rank} that with ordinal structure, the ranking method performs much better. We find that pre-training with the proposed ordinal loss significantly improves the rank consistency of these backbone networks (Appendix \ref{ap:allab}).

\begin{figure}[htbp]
  \centering
  \includegraphics[height=5.0cm,width=0.92\textwidth]{images/fasterrcnn_rank_v4.pdf}
  \caption{$CorLoc$ (\%) comparison with ranking method using Faster RCNN pre-trained backbone.}
  \label{fig:faster_rank}
\end{figure}


%Another experiment is to train an agent using embedding without ordinal structure as reward. Figure. \ref{fig:sample} ("AE+Embed") and Table \ref{tab:fasternoord} both indicate the necessity of ordinal embedding.

In contrast, being able to learn across different images, the RL localization agent shows more tolerance to the defects of the reward function. We analyze the benefits of RL component. From both Figure \ref{fig:faster_rank} and Figure \ref{fig:imgnet_rank}, when using ordinal embedding, the model with RL is generally better than ranking, especially after adaptation. 

Ordinal component is necessary for several possible reasons. First, the ordinal component makes the generic pre-trained network more specific to the downstream object localization task. Second, it helps remove the dataset bias if the pre-trained network is non-native. Third, ordinal pre-training encourages the reward signal to reflect step-by-step improvements. 

Encouraged by the strong baseline performance of Faster RCNN on both source and target domain (detailed in Table \ref{tab:fastersource} and Table \ref{tab:fastfinetune}), we investigate whether it is adequate to use Faster RCNN embedding in the RL reward function, with or without ordinal pre-training. 
Since Faster RCNN emebedding is also trained for object localization on the COCO dataset, it can separate out the effects of the ordinal pre-training component better. 
The result are shown in Table \ref{tab:fasternoord}. It can be seen that without ordinal pre-training, the performance degrades significantly and the $CorLoc$ is much lower even in source domain. More results of different backbones are presented in Appendix Table \ref{tab:backbonesource} and Table \ref{tab:backbonetarget}, from which the test-time adaptation still brings a large margin of improvement.  

\begin{table}[!h]
\centering
\caption{$CorLoc$ (\%) RL with Faster RCNN embedding w/ and w/o ordinal pre-training on source domain.}
\begin{tabular}{lccccc}
\toprule
method       & cow & cat & dog & horse & zebra  \\
\midrule
Faster RCNN backbone  & 25.93 & 13.17 & 12.16 & 16.18 & 28.57 \\
Faster RCNN backbone + Ord & \textbf{66.67} & \textbf{72.46} & \textbf{61.59} & \textbf{60.29} & \textbf{71.25} \\
\bottomrule
\end{tabular}
\label{tab:fasternoord}
\end{table}

% ################################################

% \subsubsection{Selective localization.}



% \begin{table}[hbpt]
% \centering
% \caption{Performance of loose to tight annotated bounding box.}
% \begin{tabular}[t]{lcr}
% \toprule
% Dataset & Adaptation & $CorLoc (\%)$   \\
% \midrule
% \multirow{ 2}{*}{mnist} & & 87.52 \\
% & \checkmark & 100. \\
% \midrule
% \multirow{ 2}{*}{CUB} & & 83.67 \\
% & \checkmark & 87.76 \\
% \bottomrule
% \end{tabular}
% \label{tab:trs}
% \end{table}%


% \begin{minipage}{\textwidth}
% \begin{minipage}[b]{0.49\textwidth}
% \centering
% \rule{6.4cm}{3.6cm}
% \captionof{figure}{A table beside a figure}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.49\textwidth}
% \centering
% \begin{tabular}[t]{lcr}
% \toprule
% Dataset & Adaptation & $CorLoc (\%)$   \\
% \midrule
% \multirow{ 2}{*}{mnist} & & 87.52 \\
% & \checkmark & 100. \\
% \midrule
% \multirow{ 2}{*}{CUB} & & 83.67 \\
% & \checkmark & 87.76 \\
% \bottomrule
% \end{tabular}
% \label{tab:trs}
%   \captionof{table}{A table beside a figure}
% \end{minipage}
% \end{minipage}

% ################################################

% {\color{cyan}
% \begin{enumerate}
% \item CUB: Change class/background
% \item Selective Localization: MNIST
% \item Annotation Refinement MNIST, CUB: Body to Head
% \item Few-shot: Omniglot or CUB
% \item Progressive/Continual Learning
% \item Pretrain vs joint training 
% \item Assess and Improve annotation quality
% \item \textbf{Body to head: CUB}
% \item \textbf{Few-shot: Omniglot or CUB}
% One prototype, per-class prototype, or clustering/data partition

% \item Change background: CUB
% \item The effects of Embedding (AE, Pretrain, Classification)
% \item The effects of support set
% \end{enumerate}}



% \begin{table}[ht]
% \tiny
% \setlength{\tabcolsep}{2pt}
% \centering
% \caption{Performance of Ord on different digits.}
% \begin{tabular}[t]{lccccccccccc}
% \toprule
% & 4 & 0 & 1 & 2 & 3& 5 & 6 & 7 & 8 & 9 & mean   \\
% \midrule
% Ord Inst & 92.97$$2.0 & 91.94$$0.7 & 90.31$$2.9 & 92.05$$1.8 & 91.98$$0.2 & 92.71$$0.6 & 92.59$$0.2 & 90.66$$0.7 & 91.99$$0.7 & 90.49$$0.7 & 91.64$$0.5 \\
% Ord Proto   & 92.67$$1.7 & 90.31$$0.3 & 89.07$$0.4 & 90.99$$1.1 & 90.30$$0.4 & 91.59$$0.6 & 91.44$$0.6 & 89.88$$1.5 & 91.17$$1.1 & 89.99$$0.8 &90.53$$0.4 \\
% Ord Other Inst  & 92.36$$0.3 & 89.39$$0.9 & 86.78$$0.3 & 90.02$$1.5 & 90.50$$1.2 & 90.47 $$1.2 & 90.50$$0.4 & 88.23$$0.7 & 90.45$$1.4 & 89.10$$0.2 & 89.49$$0.8 \\
% Ord Other Proto  & 92.46$$0.8 & 89.39$$0.6 & 88.19$$3.0 & 90.79$$2.2 & 90.30$$1.2 & 90.70$$0.4 & 91.13$$1.8 & 89.30$$0.9 & 90.76$$0.5 & 89.30$$0.7 & 89.98$$0.7 \\
% \bottomrule
% \end{tabular}
% \label{tab:trs}
% \end{table}%



% \begin{table}[t]
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \vskip -0.15in
%          \caption{Compare random sampling and anchor sampling on \emph{OrdAcc} (\%). }
%         \label{tab:smp}
%       \begin{tabular}[b]{lcc}
%         \toprule
%         Method &  Random & Anchor \\
%         \midrule
%         \emph{OrdAcc} (\%) & 90.12 & 92.97 \\
%         \bottomrule
%         \end{tabular}
%     \end{minipage}
%         \hfillx
%         \begin{minipage}{0.5\textwidth}
%             \centering
%               \label{tab:sign}
%             \caption{Compare with and without sign for IoU reward on \emph{CorLoc} (\%).}
%           \begin{tabular}[b]{lcr}
%             \toprule
%             Sign & Digit 4 & Other digits    \\
%             \midrule
%             \checkmark & 90.92 & 82.43 \\
%             & 94.36 & 88.64 \\
%             \bottomrule
%             \end{tabular}
%         \end{minipage}
% \end{table}

==> ICLR2022_Policy Adaptation_Final/introduction.tex <==
% 1. Choose relevant source-target for transfer learning, more explainable 
% 2. Domain-specific, not many classes available 


% Background, Scope, and Contributions
%There is increasingly interest in designing models  that can be adapted to unseen environments or repurposed for new tasks,  with only minimal human guidance \citep{vinyals2016matching, snell2017prototypical, finn2017model,  sun2020test, hansen2021selfsupervised}. A small set of examples can not only serve the purpose of implicitly generalizing the trained model to the new environment during training time, but also provide the chance of updating the learning objectives with the learner during test-time. 
There is increasing interest in designing machine learning models  that can be adapted to unseen environments or repurposed for new tasks,  with only minimal human guidance \citep{vinyals2016matching, snell2017prototypical, finn2017model,  sun2020test, hansen2021selfsupervised}. To this end, a small set of examples can not only serve the purpose of implicitly generalizing a trained model to a new environment during training time, but also enable the learner to update its learning objectives during test time. 

% the purpose of exposing the trained model to the new environment

%In this paper, we focus on the reinforcement learning (RL) formulation to the problem of \emph{query object localization}, where an agent is trained to localize the target object specified by a small set of exemplary images. {\color{blue}Instead of using fixed bounding box proposals}, the vision-based agent can be viewed as a proactive information gatherer \citep{guo2003decision} that actively interacts with the image environment, following a class-specific localization policy, thus will be more suitable for aerial imagery \citep{xia2018dota}, robotic manipulation \citep{kalashnikov2018scalable}, or embodied AI  \citep{savva2019habitat} tasks.  
In this paper, we focus on a reinforcement learning (RL) formulation to the problem of \emph{query object localization}, in which an agent is trained to localize the target object specified by a small set of exemplary images. Instead of using fixed bounding box proposals, our vision-based agent can be viewed as a proactive information gatherer \citep{guo2003decision}, which actively interacts with an image environment; Furthermore, it follows a class-specific localization policy, and thus is more suitable for aerial imagery \citep{xia2018dota}, robotic manipulation \citep{kalashnikov2018scalable}, or embodied AI  \citep{savva2019habitat} tasks. 
% than supervised counterparts \citep{redmon2016you, ren2016faster, carion2020end}

%During test-time, the queried object class to localize may be novel, or the background environment may undergo substantial change, hindering the applicability of class-agnostic agents with fixed policy. When reward signal is available, fine-tuning methods \citep{julian2020never} can effectively adapt agents to the new environment and yield improved performance. Different with standard RL settings, in object localization the reward signal is not available during test-time, as the bounding box annotations are to be found by the localization agent on test images.
During the test time of query object localization, the queried object class to localize may be novel, or the background environment may undergo substantial changes, hindering the applicability of class-agnostic agents with a fixed policy. In addition, in standard RL settings for object localization, the reward signal is often available, so fine-tuning methods \citep{julian2020never} can effectively adapt agents to new environments and yield improved performance; On the contrary, in query object localization, the reward signal is not available at test time, because the bounding box annotations are to be found by the localization agent on test images.


%To address this problem, we propose an ordinal metric learning based framework for learning an implicitly transferable reward signal defined with a small exemplary set. An ordinal embedding network is pre-trained with data augmentation under a loss function designed to be relevant to the RL task. The reward signal allows explicit updates of the controller in the policy network with continual training during test-time. Compared to fine-tuning approaches, the agents can get exposed to the new environment more extensively with unlimited usage of test images. Informed by the exemplary set precisely, the agent is versatile to the change of localization target.
To address these problems, we propose an ordinal metric learning based framework for learning an implicitly transferable reward signal defined with a small exemplary set. An ordinal embedding network is pre-trained with data augmentation under a loss function designed to be relevant to the RL task. The reward signal allows explicit updates of the controller in the policy network with continual training during test time. Compared to fine-tuning approaches, the agent can get exposed to new environments more extensively with unlimited usage of test images. Informed by the exemplary set precisely, the agent is adapted to the changes of the localization target.  

Our contributions in this paper are summarized as follows: (1) We propose a novel ordinal metric learning based RL framework to learn a transferable reward signal defined with a small exemplary set for query object localization; (2) Our RL framework enables test-time policy adaptation to new environments where there is no readily available reward signal; (3) Our learned transferable reward allows repurposing a trained agent from localizing one specific class to another; (4) Extensive experiments on several %{\color{red}benchmark} 
datasets demonstrate the effectiveness of our proposed approach.



% ({\color{blue}and environment? Emphasized in the sentence before.}). 

==> ICLR2022_Policy Adaptation_Final/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR2022_Policy Adaptation_Final/method.tex <==







% \begin{table}[hbpt]
%   \small{
% \caption{Breaking up the requirement on data and labels in different phases}\label{table:differences}
% \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{l|ccccc}
% {\ul \textbf{}} & {\ul Supervised training} & {\ul  Fine-tuning} & {\ul Ordinal embedding } & {\ul Agent training} & {\ul Test-Time adaptation} \\ \hline
% Image-box pairs       & \cmark       & \cmark       & \cmark       & \xmark       & \xmark       \\
% Unlabeled images       & \xmark       & \xmark       & \xmark       & \cmark      & \cmark       \\
% Exemplar images       & \xmark       & \xmark       & \cmark      & \cmark      & \cmark      
% \end{tabular}}}
% \end{table}





%For all experiments, we apply policy gradient (REINFORCE) \citep{williams1992simple} with entropy loss to encourage exploration. Similarly to \citep{mnih2014recurrent}, we consider the localization as a POMDP problem, where the agent is built around a recurrent neural network (RNN) to process inputs sequentially. Contrast to region-proposal  based methods, where they process an entire image at once, the agent selects the actions to transform current bounding box at each step. The agent takes pooled feature from the current box as \emph{State}, while it also maintains an internal state within RNN, which encodes information from history observations. \emph{Actions} are defined with discrete five scaling and eight translation transformations as in \citep{jie2016tree}, plus one stay action. 


\subsection{RL formulation for query object localization}
Given a set of images $\mathcal{I}$ with known class labels, the task of query object localization is to find the location $b$ of the bounding box most relevant to the query object, specified in a small set of exemplary images $\mathcal{E}$. Following the Markov Decision Process (MDP) framework for object localization \citep{caicedo2015active, jie2016tree}, this task can be formulated as a RL problem. In the training phase, a localization agent learns to take actions %on 
of moving the bounding box %and maximum
to maximize a reward function reflecting  localization accuracy. In the test phase, the agent is informed by a small test exemplary set about %the 
a new task objective. Figure \ref{fig:overview} shows an overview of the query object localization problem and the RL formulation, with components listed as follows.


% In query object localization, we are given a set of images $\mathcal{I}$,  and a small set of exemplary images $\mathcal{E}$.  Our goal is to find the location $b$ of the bounding box  containing the queried object in each image. 


% Reward signal defined on an exemplary set with preference encoded in the ordinal representation. Policy trained and adapted to a new class.Target object is specified  by query images in the exemplary set

% \begin{figure}[!h]
%   \centering
%   \includegraphics[height=3.5cm,width=0.9\textwidth]{images/fig1.png}
%   \caption{Illustration of few shot object localization. }
%   \label{fig:1}
% \end{figure}


% Training test, exemplary with environment. Test time, can be only exemplary set without environment. 
 
\begin{itemize}
    \item \textbf{Environment:} Raw pixels of a single image $I_{i}$,  without candidate proposal boxes. 
    \item \textbf{Action:} Discrete actions facilitating a top-down search, including five scaling: scale towards top left/right, bottom left/right, center; eight translation transformations: move left/right/up/down, enlarge width/height, reduce width/height; plus one stay action. 
    \item \textbf{State:} Pooled features from the current box and an internal state within RNN %, which 
    that encodes information from history observations. 
    \item \textbf{Reward:} Improvements the agent made in localizing the query images (in different tasks). 
\end{itemize}


% , while it also maintains an internal state within RNN, which encodes information from history observations. 

% we consider raw pixels in each image $I_{i}$ as the \emph{\textbf{Environment}}.  
% we define \emph{\textbf{Action}} set with discrete actions facilitating a top-down search, including five scaling, eight translation transformations as in \citep{jie2016tree}, plus one stay action. 


% The agent takes pooled feature from the current box as \emph{\textbf{State}}, while it also maintains an internal state within RNN, which encodes information from history observations. 

\subsection{Pre-training ordinal reward signal}\label{sec: reward}


% \subsection{Learning Ordinal Reward Signal}\label{sec: reward}
% % \subsection{Ordinal Embedding based Reward Signal}


For training an agent to localize different objects according to 
queries, the reward function needs to be transferable.
Existing deep RL approaches for object localization \citep{caicedo2015active, jie2016tree} use its ground-truth object bounding box $g_{i}$ as the reward signal, 
\begin{align}\label{IoU: reward}
    R = \textrm{sign}(\textrm{IoU}(b_t, g_i)-\textrm{IoU}(b_
    {t-1}, g_i)), 
\end{align}
where $\textrm{IoU}(b_t, g_i)$ denotes the Intersection-over-Union (IoU) between the current window $b_t$ and the corresponding ground-truth box $g_i$\footnote{Bounding box are denoted by lowercase lightface letters, e.g., $g$, while embedding vectors are denoted by boldface letters, e.g., $\mathbf{g}\in \mathbb{R}^{d}$ is a $d$-dimensional vector. }, and $\textrm{IoU}(b, g) = \textrm{area}(b \cap g)/\textrm{area}(b\cup g)$. Similar to the bounding box regression approaches which learn a mapping ${\color{black}\phi}: I\mapsto g$, the image and box must be paired. However, annotated image-box pairs $(I, g)$ may be scarce in both the training and testing phases. The reward signal %in Eq. \ref{IoU: reward} is defined instance-wise,
defined in Eq.~\ref{IoU: reward} is instance-wise, which is not transferable across images. 

% is not transferable across training images, not to mention test image with potential domain shifts. 

To address this problem, a natural idea is to define the reward signal based on learned representations %between 
of the cropped images by current window $b_t$ %,
and the ground-truth window $g$. Given their $M$-dimensional representations $\mathbf{b_t}$ and $\mathbf{g}$ produced by an embedding function ${\color{black}f}: \mathbb{R}^{D}\mapsto \mathbb{R}^{
M}$ from $D$- dimensional image feature vectors, a distance function $d: \mathbb{R}^{M}\times \mathbb{R}^{M} \mapsto [0, +\infty)$ %return 
returns the embedding distance  $d(\mathbf{b_t}, \mathbf{g})$. However, an embedding distance based on off-the-shelf pre-trained networks %are 
is not adequate, since it may not decrease monotonically as the agent approaches to the ground-truth box $g$. As a result, the embedding distance based reward signal may be less effective than Eq. \ref{IoU: reward} (as shown in Section \ref{sec:experiment}). Therefore, an embedding function customized for the downstream RL-based localization task is needed.     

\textbf{Ordinal metric learning.}  We propose to use an ordinal embedding based reward signal. For any two perturbed boxes $b_j, b_k$ from ground truth $g$, embeddings $\mathbf{b_{j}},\mathbf{b_{k}}, \mathbf{g}$ are learned, such that the relative preferences between any pair of boxes are preserved in the Euclidean space, 
\begin{align}\label{eq: ordinal}
\rho_{j}>\rho_{k}\Leftrightarrow ||\mathbf{b_j}-\mathbf{g}||<||\mathbf{b_k}-\mathbf{g}||, \quad \forall j, k \in \mathcal{C},
\end{align}
where $\rho_j$ and $\rho_{k}$ denote the preference (derived from either IoU to ground-truth box or ordinal feedback from user), and $\mathcal{C}$ is an ordinal constraint set constructed by sampling box pairs around $g$. 
This problem is originally posed as non-metric multidimensional scaling \citep{agarwal2007generalized, jamieson2011low}. Although we apply a very simple pairwise-based approach, there exist other extensions such as the listwise-based \citep{cao2007learning}, quadruplet-based \citep{terada2014local} and landmark-based \citep{anderton2019scaling, Ghosh2019} approaches. 


% {\color{red}It also makes the downstream task of policy network training more efficient.} 

\textbf{Loss function.} In this paper, we define preference $\rho$ as the IoU of box $b$ to the ground-truth box $g$, i.e., $\rho= \textrm{IoU}(b, g)$. 
We choose to optimize %the 
a triplet loss \citep{hermans2017defense} for learning the desired %embedding,
embeddings,
\begin{align}\label{eq:triplet}
\mathcal{L}_{\textrm{triplet}} = {\sum_{{\color{black}\textrm{anchor, ordinal pairs}}}} \max\big(m + d(\mathbf{a},\mathbf{p}) - d(\mathbf{a},\mathbf{n}), 0\big),     
\end{align}
where $\mathbf{a}$ is the ``anchor" embedding that will be discussed in detail later,  $\mathbf{p},\mathbf{n}$ are the ``positive" and ``negative" embeddings for boxes with larger and smaller IoUs with ground truth box $g$, respectively, $m$ is a margin hyper-parameter.  We learn an embedding space consistent with local ordinal constraints on positive and negative data   %specified on the by image-box pairs obtained 
obtained via data augmentation such as box perturbation. %This can be viewed as a procedure to enhance the robustness of neural network \citep{szegedy2014intriguing} against box perturbations, and protect the special purpose of its usage on distinguishing reward increases or decreases. 


\textbf{Box Perturbation} Assuming the training exemplary set $\mathcal{E}_{\textrm{train}}$ contains both image $I$ and box $g$, we adopt a tailored data augmentation scheme - \emph{box perturbation}, in which a pair of boxes are randomly sampled from $I$ with different IoUs to $g$. We compare the efficiency of sampling schemes on generating augmented bounding box pairs, (a) \emph{Random sampling}, where the pair of boxes are generated completely randomly, and (b) \emph{Group-based sampling}, where dense boxes with variant scales are first generated, and then divided into $M=10$ groups according to the IoU with ground-truth box. Each group has an IoU interval of $1/M$. The sampling is first done on the group level, i.e., $2$ out of $M$, then sample one box from each group. Thus, the sampled boxes are likely to cover more diverse cases comparing to random sampling.  We have found that using IoU-based partition scheme is more effective than  random sampling. 

% Using the same number of pairs, the resulting \emph{OrdAcc} for the two schemes is 90.12\% (random sampling), 92.97\% (group sampling), respectively.
% \textbf{Sampling scheme.} 
% {\color{blue}random vs. anchor?} 
 


\textbf{The choice of anchor.}
The anchor embedding $\mathbf{a}$ in Eq. \ref{eq:triplet} is not %restrictive
restricted to the cropped image from the same image. For example, it could be replaced by the prototype embedding \citep{snell2017prototypical} of the exemplary set $\mathcal{E}$, $\mathbf{c} = {1}/{|\mathcal{E}|} \sum_{i\in \mathcal{E}}\mathbf{g}_{i}$, where $\mathbf{g}_{i}$ is the embedding of the cropped image $I_{i}$ by ground-truth box $g_{i}$. If images from multiple %class
classes are of interest, the prototype can be further made to be class-dependent, or clustering-based. 
A prototype as the anchor enables test-time policy adaptation without image-box pairs in the exemplary set $\mathcal{E}_{\textrm{test}}$.  In comparison, supervised methods such as Faster RCNN would require image-box pairs for fine-tuning on new tasks. In some experiments (Appendix \ref{ap:allab}), we find that using prototype-based embedding as the anchor could lead to better generalization performance than using $\mathbf{g}$. 
It is also interesting to explore other treatment on the exemplary set, such as permutation-invariant architectures \citep{zaheer2017deep, ilse2018attention, lee2019set}.

% Even if the test exemplary set only contains the cropped object (i.e., no image-box pairs), test-time policy adaptation is still feasible.

% Moreover, even if the exemplary set during the test time only contains the cropped object, test-time policy adaptation is still feasible without image-box pairs. 
\begin{figure}[b]
\vspace{-0.5cm}
  \centering
  \includegraphics[height=0.30\textwidth,width=0.7\textwidth]{images/Fig2_v6_main.png}
  \caption{%Left:
  (a) Modules for ordinal representation learning. The RoI encoder extracts RoI feature that will be used as the state representation for localization. The projection head learns ordinal embedding $\mathbf{b}$ for computing reward.  %Right:
  (b) Controller network. In each step, the agent takes the output from the RoI encoder as state, while it also maintains an internal hidden state $h^r$ within a RNN, which encodes information from history observations. Then it outputs the action for next step.}
  \label{fig:2revision}
\end{figure}

\vspace{-0.1cm}
\subsection{Localization agent training}

As discussed in Section \ref{sec: reward}, we use the ordinal embedding rather than the bounding box coordinates to quantify the improvement that an agent makes, and the continuous-valued reward for %an
the agent moving from state $s'$ to $s$ takes the following form, \begin{align}\label{eq:4}
    R(s,s')=||\mathbf{b}_{t-1}-\mathbf{c}||-||\mathbf{b}_{t}-\mathbf{c}||, 
\end{align}
where $\mathbf{c}$ is the prototype embedding, $\mathbf{b}_{t}$ is the embedding of the cropped region at step $t$.   % Ordinal embeddings are extracted from the image regions surrounded by the ground-truth boxes in $\mathcal{E}$, by the pre-trained RoI encoder and projection head, and the protoptype is computed as the mean vector.  
We expect positive reward if the embedding distance between cropped image $\mathbf{b}_{t}$ and query image $\mathbf{a}$ is decreased.    



\textbf{State representation.}
Note that a good representation for defining reward may not necessarily be a good state representation at the same time - it may not contain enough information guiding the agent taking the right actions. 
\cite{chen2020simple} suggests that adding a projection head between the representation and the contrastive loss substantially improves the quality of the learned representation. 
We find that the use of projection head is crucial in balancing the two objectives in our task. The network architecture is shown in Figure \ref{fig:2revision}(a), in which an MLP projection head is attached after an (Region of Interest) RoI encoder. The ROIAlign module handles boxes of different sizes.

\textbf{Policy network.} Starting from %the
a whole image %pixels
as input, the agent is trained to select %the 
actions to transform the current box at each step, %by 
maximizing the total discounted reward. We use policy gradient %with 
based on a recurrent neural network (RNN) \citep{mnih2014recurrent} %rather than DeepQNetwork 
with a vector of history actions and states.  More detailed architecture can be found in Figure \ref{fig:2revision}(b) and Appendix Figure \ref{fig:encode_agent}. For all experiments, we apply policy gradient (REINFORCE) \citep{williams1992simple} with entropy loss regularization to encourage exploration. The %full
main algorithm is outlined in Algorithm \ref{alg:g-rep}.

 


% {\color{cyan}update accordingly with state representation $\mathbf{s}$ and reward embedding $\mathbf{b}$, (we use $b$ and $g$ for boxes, $\mathbf{b}$ for embeddings) if possible, simplify the notation a little bit.}






% Local ordinal constraints. Consider an image annotated with ground truth bounding box $b_{i}$. Assume there exists a dissimilarity function $\xi$. 
% , but this can not be achieved directly. 
% The learning transferable reward follows the  



% \subsection{Training Localization Agent}

\begin{algorithm}[ht]
\begin{minipage}[t]{0.99\textwidth}
\footnotesize
    \caption{Training localization agent using the proposed ordinal reward signal.}\label{alg:g-rep}
    \DontPrintSemicolon
    \SetAlgoLined
    \SetKwInOut{KwInput}{Require}
    \SetKwInOut{KwOutput}{Output}
    \KwInput{initial policy $\pi_{\theta}$, batch size $N$, pre-trained RoI encoder $e$ and projection head $h$, learning rate $\alpha$}
    \KwOutput{policy network $\pi_{\theta}$}
    \For{sampled minibatch $\left \{x_k \right \}^N_{k=1}$}{
      \For{k=1,...N}{
        %$\mathbf {x_k}\leftarrow e(x_k)$ \;
        Construct an exemplary set $\mathcal{E}_{\textrm{batch}}$ \; 
         $\mathbf{g_j}\leftarrow h(e(x_k, g_j))$ \tcp*[l]{compute the ordinal embedding in Figure 2(a)}
        $\mathbf{c}_{k}\leftarrow\frac{1}{\left | \mathcal{E}_{\textrm{batch}} \right |}\sum_{j \in \mathcal{E}_{\textrm{batch}}} \mathbf{g}_{j}$ \tcp*[l]{compute the prototype vector} 
        $\tau _k\leftarrow\left \{\ s_1, a_1, ...s_T, a_T \right \}$ by running policy $\pi_{\theta}$\tcp*[l]{sample trajectory}
        $\mathbf{b_t}\leftarrow$ take action $a_t$, and compute embedding $h(e(x_k, b_t))$ for current window $b_{t}$ \;
        $R_{k}^{t}\leftarrow\left \| \mathbf{b}_{t-1}-\mathbf{{c}}_{k} \right \|-\left \| \mathbf{b}_t-\mathbf{{c}}_{k} \right \|$ \tcp*[l]{compute reward in equation 4}
        
      }
      $\theta \leftarrow \theta +\alpha \nabla _{\theta}\sum_{k=1}^{N}\left [ \log\pi _{\theta} \left (  \sum_{t'=t}^{T}\gamma ^{t'-t}R_{k}^{t}\right )- \lambda \cdot \pi _{\theta}\log\pi _{\theta}\right ]$ \tcp*[l]{policy update}
     }
     \end{minipage}
\end{algorithm}
% \vspace{-0.5cm}
\subsection{Test-time adaptation}


During %test-time
test time, the agent has the option of further updating the policy network using the received reward from Eq. \ref{eq:4}. To match test conditions, the training batch is split into two %group
groups, and $\mathbf{c}$ is computed on a small subset that does not overlap with the training images to localize; %, while during
During test-time adaptation, $\mathbf{c}$ becomes the prototype of the test exemplary set $\mathcal{E}_{\textrm{test}}$. Different from $\mathcal{E}_{\textrm{train}}
$, only cropped images are needed in $\mathcal{E}_{\textrm{test}}
$ as shown in Figure~\ref{fig:overview}.   

% {\color{cyan}[entropy is important; Reward $\{+1, -1\}$, ours $\mathbb{R}$? How to terminate, Deep]}
% In training stage, before the agent starts to localize, the RoI encoder and projection head first extracts the ground-truth RoI ordinal embedding, noted as $f^{ord}_{gt}$. Then the agent learns to localize, by comparing the embedding of the predicted bounding box and the ground-truth. For each step, the agent takes the RoI feature as state, and predict an action to generate a new RoI for encoder. The learning objective is to maximize the total discounted reward.

% We formulate localization as Markov Decision Process (MDP) as in \citep{caicedo2015active, jie2016tree}, where the agent is built around a recurrent neural network (RNN) to process inputs sequentially. It is trained to select the actions to transform current bounding box at each step, by maximizing the total discounted reward. The agent takes pooled feature from the current box as \emph{State}, while it also maintains an internal state within RNN, which encodes information from history observations. \emph{Actions} are defined with discrete five scaling and eight translation transformations as in \citep{jie2016tree}, plus one stay action. To match test conditions, the \emph{Reward} is defined as 
% \begin{equation}
%     R(s,s')=||\mathbf{b_{t}}-\mathbf{a}||-||\mathbf{b_{t'}}-\mathbf{a}||
% \label{eq:4}
% \end{equation}
% where $\mathbf{a}$ is a small subset within a batch that doesn't contain this instance. While during adaptation stage, $\mathbf{a}$ becomes the prototype of the exemplary set. 

% The framework of our method is represented in Fig.\ref{fig:3}. Our model is composed of RoI encoder, projection head and an agent. The RoI encoder is to extract RoI feature according to the given image and RoI (Region of Interest). The projection head is to learn ordinal embedding for reward. And the agent is to learn localization. In training stage, before the agent starts to localize, the RoI encoder and projection head first extracts the ground-truth RoI ordinal embedding, noted as $f^{ord}_{gt}$. Then the agent learns to localize, by comparing the embedding of the predicted bounding box and the ground-truth. For each step, the agent takes the RoI feature as state, and predict an action to generate a new RoI for encoder. The learning objective is to maximize the total discounted reward .







% \begin{algorithm}[t]
% \begin{minipage}[t]{0.99\textwidth}
% \footnotesize
%     \caption{Training localization agent using the proposed ordinal reward signal.}\label{alg:g-rep}
%     \DontPrintSemicolon
%     \SetAlgoLined
%     \SetKwInOut{KwInput}{Input}
%     \SetKwInOut{KwOutput}{Output}
%     \KwInput{initial policy $\pi_{\theta}$, examplary set size $s$, batch size $N$, pre-trained $e$ and $h$, learning rate $\alpha$}
%     \KwOutput{policy controller $\pi_{\theta}$}
%     \For{sampled minibatch $\left \{x_k \right \}^N_{k=1}$}{
%       \For{k=1,...N}{
%         %$\mathbf {x_k}\leftarrow e(x_k)$ \;
%         \uIf {training}{
%             $\mathbf{g_k}\leftarrow h(e(x_k, g_k))$ \;
%             $\mathbf{g'_k}\leftarrow$ random shuffle $\mathbf{g_k}$  \;
%             $\mathbf{c_{m}}=\frac{1}{\left | S_m \right |}\sum_{\mathbf{g'_j}\in S_m}\mathbf{g'_j}$, $m=1,...\lfloor N/s \rfloor$\;
%         }
%         \uElseIf{adaptation}{ compute the prototype embedding: 
%         $\mathbf{\bar{q}}=\frac{1}{\left | \mathcal{E}_{\textrm{test}} \right |}\sum_{j \in \mathcal{E}_{\textrm{test}}} \mathbf{q_j}$ \;
%         }
%         % sample trajectory $\tau _k=\left \{\ s_1, a_1, ...s_T, a_T \right \}$ by running policy $\pi_{\theta}$\;
%         $\mathbf{b_t}\leftarrow$ take action $a_t$, and compute embedding $h(e(x_k, b_t))$ \;
%         \uIf {training}{
%         $R_{k}^{t}=\left \| \mathbf{b_{t-1}}-\mathbf{c_m} \right \|-\left \| \mathbf{b_t}-\mathbf{c_m} \right \|$\;
%         }
%         \uElseIf{adaptation}{
%         $R_{k}^{t}=\left \| \mathbf{b_{t-1}}-\mathbf{\bar{q}} \right \|-\left \| \mathbf{b_t}-\mathbf{\bar{q}} \right \|$\;
%         }
%       }
%       $\theta \leftarrow \theta +\alpha \nabla _{\theta}\sum_{k=1}^{N}\log\pi _{\theta} \left (  \sum_{t'=t}^{T}\gamma ^{t'-t}R_{k}^{t}\right )$ \tcp*[l]{policy update}
%      }
%      \end{minipage}
% \end{algorithm}



% \begin{algorithm}[bpht]
%     \DontPrintSemicolon
%     \SetAlgoLined
%     \SetKwInOut{KwInput}{input}
%     \SetKwInOut{KwOutput}{output}
%     \KwInput{{\color{red}Input images \mathcal{I}, exemplary set $\mathcal{E}$? } batch size N $\bx$}
%     \KwOutput{agent $q$ $\bv$}
%     pre-train RoI encoder $f$ and projection head $h$ $\bv$\;
%     {\color{gray}\# \textit{training}} $\bv$\;
%     \For{sampled mninibatch $\left \{\mathbf{x_k}\right \}^N_{k=1}$}{
%       Compute ground-truth reward embedding $\left \{\mathbf{g_{k}}\right \}\in \mathbb{R}^{M\times N}$ $\bv$\;
%       Shuffle and group $\left \{\mathbf{g_{k}}\right \}\in \mathbb{R}^{M\times N}$ to $\left \{\mathbf{g'_{k}}\right \}\in \mathbb{R}^{M\times N'}$ $\bv$\;
%       Apply $f$ and $q$ to get policies $\left \{\pi_k^t\right \}\in \mathbb{R}^{T\times N}$ $\bv$\;
%       Compute rewards $\left \{r_{k}^{t}\right \}\in \mathbb{R}^{T\times N}$ using \eqref{eq:4}, where ${\mathbf{a}}=\mathbf{g'_{k}}$ $\bv$\;
%       Get accumulated rewards $\left \{R_k^{t}\right \}\in \mathbb{R}^{T\times N}$ $\bv$\;
%       Normalize $\left \{R_K^{t}\right \}$ to $\left \{\bar{R}_{k}^{t}\right \}$ $\bv$\;
%       Call the gradient ascent $\sum \left \{\bar{R}_{k}^{t}log\pi _{k}^{t}\right \}$ $\bv$\;
      
%      % }
%      }
%      {\color{gray}\# \textit{adaptation}} $\bv$\;
%      Compute prototype embedding $\mathbf{\bar{g}}=\frac{1}{S}\sum \mathbf{g_{k}}$ of examplary set $\bv$\;
%      \For{sampled mninibatch $\left \{\mathbf{x_k}\right \}^N_{k=1}$}{
%       repeat {\color{red}step 6 to step 10}, except $\mathbf{a}=\mathbf{\bar{g}}$   $\bv$\;
%      }
%     \caption{Training reward and localization agent\label{alg:g-rep}}
% \end{algorithm}

% \begin{algorithm}[bpht]
%     \DontPrintSemicolon
%     \SetAlgoLined
%     \SetKwInOut{KwInput}{input}
%     \SetKwInOut{KwOutput}{output}
%     \KwInput{data $\bx$, probabilistic model $p(\bx,\bz)$, variational family $q(\bz;\bv)$, transformation $\bz=\Tcal(\beps;\bv)$}
%     \KwOutput{variational parameters $\bv$}
%     Initialize $\bv$\;
%     \Repeat{convergence}{
%       Draw a single sample $\bz\sim q(\bz;\bv)$\;
%       Compute the auxiliary functions $\hfun\left(\Tcal^{-1}(\bz;\bv);\bv\right)$ and $\ufun\left(\Tcal^{-1}(\bz;\bv);\bv\right)$ (Eq.~\ref{eq:hfun_ufun})\;
%       Estimate $\bg^{\textrm{rep}}$ and $\bg^{\textrm{corr}}$ (Eq.~\ref{eq:grep_gcorr}, estimate the expectation with one sample)\;
%       Compute (analytic) or estimate (Monte Carlo) the gradient of the entropy, $\nabla_{\bv}\ent{q(\bz;\bv)}$\;
%       Compute the noisy gradient $\nabla_{\bv}\Lcal$ (Eq.~\ref{eq:corrected_reparam})\;
%       Set the step-size $\brho^{(i)}$ (Eq.~\ref{eq:step_schedule}) and take a gradient step for $\bv$\; % (Eq.~\ref{eq:v_new})\;
%     }
%     \caption{Training reward and localization agent\label{alg:g-rep}}
% \end{algorithm}

% \begin{figure}[!t]
%   \centering
%   \includegraphics[height=5cm,width=\textwidth]{images/fig2.png}
%   \caption{Framework of the proposed method.}
%   \label{fig:3}
% \end{figure}



% Bounding box vs embedding distance 




% use exemplary set as a guidance signal for deliver learning objectives 

% use test image environment to expose the agent to the domain shifts 

% taking raw image pixel as input

% entropy is important 

% How to terminate

% support set - with annotations 
% prediction set - without annotations 
% customized to a different purpose 
% re-purposed 

% \subsection{Toward Adaptation to Novel Tasks}
% We explore the possibility of using our framework to repurpose the trained agent to a novel task during the test-time.  A task is considered as \emph{novel} if its learning objective potentially conflicts with the trained objective. We consider {\color{red}two} experiments in below (full details in Appendix).  

% \begin{figure}[bpht]
%   \centering
%   \includegraphics[height=5.5cm,width=0.975\textwidth]{images/body.png}
%   \caption{Visualization of bird localization}
%   \label{fig:body}
% \end{figure}




% \begin{figure}[hbpt]
% \centering
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/head0.png}
%   \label{fig:loc4}
% \end{subfigure}%
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/head5.png}
%   \label{fig:locg}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/head2.png}
%   \label{fig:locg}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/head_fail.png}
%   \label{fig:loc4}
% \end{subfigure}%
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/head2_fail.png}
%   \label{fig:locg}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/head3_fail.png}
%   \label{fig:locg}
% \end{subfigure}
% \caption{Evaluate transferring to localize head with agent trained to localize entire body. First row: successful cases, second row are failure cases.}
% \label{fig:heads}
% \end{figure}




% ################################################

%  {\color{red}During experiments, we have also found that localizing small objects (e.g., bird heads) can be more difficult}. 
%  Admittedly, the fast adaptation ability of the agent may also make it vulnerable to misleading guidance. Possibly a "safeguard" dataset is needed to make sure the agent is working as expected without negative societal impacts.
% Our algorithm takes raw image pixels as input with no need of proposing candidate boxes. 

% Or given two similar objects coexisting in one image environment, can we train the agent to pick up one from the two during the training test, while adapt it to pick another one during the testing?   We consider a two-digits environment with random patch background noise. Different from unsupervised approaches \citep{wei2017deep}, which mostly relies on low-level images clues to distinguish foreground and background, we can specify it using the exemplary set. The exemplary sets used in training and testing are switched, therefore the agent is asked to localize different digits. 




% \subsection{Discussions}\label{sec: limitations} 


==> ICLR2022_Policy Adaptation_Final/related_work.tex <==
% How to do object localization?
% \vspace{-0.2cm}
\subsection{Object localization}
% \paragraph{Object localization.}
Compared to bounding-box regression approaches \citep{redmon2016you, ren2016faster}, deep RL based object localization approaches \citep{caicedo2015active, jie2016tree} have the advantage of being region-proposal free, with customized search paths %to 
for each image environment. The specificity of an agent purely depends on the classes of bounding-boxes used in the reward. They can be made class-specific \citep{caicedo2015active}, but the agent for each class would need to be trained separately.
% {\color{blue}what does isolation mean?}

Despite the rise of crowdsourcing platforms, obtaining ample amount of bounding-box annotations remains costly and error-prone. Furthermore, the quality of annotations often varies, and precise annotations for certain object class may require special expertise from annotators. The emergence of weakly supervised object localization (WSOL) \citep{song2014learning, oquab2015object, zhou2016learning} methods alleviates the situation,  %which utilize image class labels in deriving bounding box annotations.
in which image class labels are used to derive bounding box annotations. It is known that WSOL methods have drawbacks of overly relying on %the
inter-class discriminative features and %not being able 
failing to generalize to classes unseen during the training phase. 

We argue that intra-class similarity is a more natural objective for the problem of localizing objects belonging to %the 
a target class. %The name 
"Query object localization" emphasizes more about the class-specific nature of %the 
a localization task, with the relevance defined by the similarity to %the 
query images. A similar problem is image co-localization \citep{tang2014co, wei2017deep}, %where 
in which the task is to identify the common objects within a set of images. Co-localization approaches exploit the common characteristics across images to localize objects. Being unsupervised, co-localization approaches could suffer from ambiguity if there exist multiple common objects or parts, e.g., bird head and body \citep{jaderberg2015spatial}, which may provide %the 
unwanted common objects as output.  

\begin{figure}[b]
\vskip -0.15in
\begin{center}
\tiny{$
\begin{array}{c}
% \hspace{-0.5cm}
 \includegraphics[height=0.30\textwidth, width=0.65\textwidth]{images/fig1_revision.png}
% &\includegraphics[height=0.21\textwidth, width=0.4\textwidth]{images/Fig1_b.png}
% \\(a) \textrm{ Skew-Normal} (\alpha = 5)& (b)\textrm{ Student's t } (\nu = 1)
\end{array}$}
\end{center}
%\vskip -0.15in
%\setlength{\belowcaptionskip}{-20.5pt}
\caption{RL-based query object localization: training and adaptation. Image-box pairs are only available in the training phase. Test environments include images without box annotations and an exemplary set specifying %changed 
a different task objective. Thus, the trained policy needs to be adapted.
}\label{fig:overview}
%\vskip -0.00in
\label{fig:1}
\end{figure}
% meta pixel-wise similarity, sensitive to the classification
% lost the specificity
% \vspace{-0.2cm}

\subsection{Policy adaptation}
% \paragraph{Policy adaptation.}

% Pretraining, support set, and fine-tuning 
% For better generalization upon domain shift, Transfer knowledge from data-abundant to data-scarce tasks
% Inform the change 
% For more precise, deambiguity of the learning goal 
There seems to be a contradiction between the goals of training an agent with high task-specificity and better generalization performance to new situations at the same time. The key to reconcile these two goals lies in the usage of a small set of examples. There has been a paradigm shift from training static models defined with parameters to dynamic ones defined together with a support set \citep{vinyals2016matching, snell2017prototypical}, proved to be very effective in few-shot classification. 

%Besides the effort of meta learning implicitly adjustable models,
Besides the efforts of employing meta learning to adjust models, fine-tuning on a pre-trained model \citep{oquab2014learning, finn2017model, julian2020never} has also been widely used in transferring knowledge from data-abundant to data-scarce tasks. When reward signal is not available, \citep{hansen2021selfsupervised}  proposed a policy adaptation approach, in which the intermediate representation is fine-tuned via optimizing a self-supervised auxiliary loss while the controller is kept fixed. Our work shares the same motivation of test-time training \citep{sun2020test}, but we focus instead on the settings where the controller needs to be adapted or even repurposed for new tasks. 

% Class-agnostic approaches neglect the difference between categories, pool all data together.  







